Towards Practical Fabrication Stage Attacks Using Interrupt-Resilient Hardware Trojans

We introduce a new class of hardware trojans called interrupt-resilient trojans (IRTs). Our work is motivated by the observation that hardware trojan attacks on CPUs, even under favorable attack scenarios (e.g., an attacker with local system access), are affected by unpredictability due to non-deterministic context switching events. As we confirm experimentally, these events can lead to race conditions between trigger signals and the CPU events targeted by the trojan payloads (e.g., a CPU memory access), thus affecting the reliability of the attacks. Our work shows that interrupt-resilient trojans can successfully address the problem of non-deterministic triggering in CPUs, thereby providing high reliability guarantees in the implementation of sophisticated hardware trojan attacks. Specifically, we successfully utilize IRTs in different attack scenarios against a Linux-capable CPU design and showcase its resilience against context-switching events. More importantly, we show that our design allows for seamless integration during fabrication stage attacks.We evaluate different strategies for the implementation of our attacks on a tape-out ready high-speed RISC-V microarchitecture in a 28nm commercial technology process and successfully implement them with an average overhead delay of only 20 picoseconds, while leaving the sign-off characteristics of the layout intact. In doing so, we challenge the common wisdom regarding the low flexibility of late supply chain stages (e.g., fabrication) for the insertion of powerful trojans. To promote further research on microprocessor trojans, we open-source our designs and provide the accompanying supporting software logic.

==> sections/section_4/irt_hmodules_cpuevents.tex <==
\begin{table*}
%\minipage[b]{1\linewidth}
\centering
%\subfloat[\scriptsize{CPU modules influenced from values of executed instructions.}]{
\captionsetup{justification=centering}
\subcaptionbox{\scriptsize{Suitable CPU host modules for IRT-2.}}{
\begin{tabular}[b]{c}
    \toprule
    \textbf{\shortstack{Attacker Influenced\\CPU Modules}}\\
    \midrule
    Adders \textcolor{ForestGreen}{\checkmark}\\
    Dividers\\
    Multipliers\\
    Floating Point Registers\\
    General Purpose Registers\\
    %Translation Lookaside Buffers\\
    \bottomrule
\end{tabular}
\label{table:cpu_attacker_infl}
}
%}
%\caption{CPU modules that can be influenced by an attacker in a microarchitecture.}
%\vspace{-2em}
\quad
%\hfill
% \subfloat[\scriptsize{CPU modules supporting context switching operations.}]{
\captionsetup{justification=centering}
\subcaptionbox{\scriptsize{Suitable CPU host modules for IRT-1.}}{
\begin{tabular}[b]{c}
    \toprule
    \textbf{\shortstack{Attacker Influenced CPU Modules\\Restoring Architectural State}}\\
    \midrule
    Program Counter\\
    Floating Point Registers\\
    General Purpose Registers \textcolor{ForestGreen}{\checkmark}\\
 %   \toprule
%   \textbf{Modules Restoring Microarchitectural State}~\cite{patent:9361101}\\
%    \midrule
%    \nassos{Reorder Buffers}\\
%    \nassos{Retirement Registers}\\
%    \nassos{Performance Monitoring Counters}\\
    \bottomrule
\end{tabular}
\label{table:cpu_state_restore}
}
%\caption{\scriptsize{CPU modules supporting context switching operations.}}
%}
%
%\vspace{-2em}
%\label{table:cpu_state_restore}
%\caption{the one for all}
\quad
%\hfill
% \subfloat[\scriptsize{CPU events lasting multiple clock-cycles.}]{
\captionsetup{justification=centering}
\subcaptionbox{\scriptsize{CPU events lasting multiple clock-cycles.}}{
\begin{tabular}[b]{c}
    \toprule
    \textbf{\shortstack{Time Expensive Events\\(Microarchitecture Dependent)}}\\
    \midrule
    Number Division\\
    Page Table Walking \textcolor{ForestGreen}{\checkmark}\\
    Branch Missprediction\\
    Missaligned Memory Accesses\\
    Translation Lookaside Buffer Flush\\
    \bottomrule
\end{tabular}
\label{table:cpu_time_expensive}
}
%}
%\caption{}
%\vspace{-2em}
%\label{table:cpu_time_expensive}
%\endminipage
\captionsetup{justification=centering}
\caption{Modules and CPU events for supporting IRTs. \\The  \textcolor{ForestGreen}{\checkmark} symbol denotes the examples we used in our implementation.}
\label{table:cpu_tables}
\end{table*}

==> sections/section_5/cs_fs_solutions.tex <==
\begin{table*}
%\minipage[b]{1\linewidth}
\centering
% \subfloat[\scriptsize{CPU events lasting multiple clock-cycles.}]{
\subcaptionbox{\scriptsize{CPU events lasting multiple clock-cycles.}}{
\begin{tabular}[b]{c}
    \toprule
    \textbf{\shortstack{Time Expensive Events\\(Microarchitecture Dependent)}}\\
    \midrule
    Number Division\\
    Page Table Walking \textcolor{ForestGreen}{\checkmark}\\
    Branch Missprediction\\
    Missaligned Memory Accesses\\
    Translation Lookaside Buffer Flush\\
    \bottomrule
\end{tabular}
\label{table:cpu_time_expensive}
}
%}
%\caption{}
%\vspace{-2em}
%\label{table:cpu_time_expensive}
\quad
%\hfill
% \subfloat[\scriptsize{CPU modules supporting context switching operations.}]{
\subcaptionbox{\scriptsize{CPU modules supporting context switching operations.}}{
\begin{tabular}[b]{c}
    \toprule
    \textbf{Modules Restoring Architectural State}\\
    \midrule
    Program Counter\\
    Floating Point Registers\\
    General Purpose Registers \textcolor{ForestGreen}{\checkmark}\\
    \toprule
    \textbf{Modules Restoring Microarchitectural State}~\cite{patent:9361101}\\
    \midrule
    Reorder Buffers\\
    Retirement Registers\\
    Performance Monitoring Counters\\
    \bottomrule
\end{tabular}
\label{table:cpu_state_restore}
}
%\caption{\scriptsize{CPU modules supporting context switching operations.}}
%}
%
%\vspace{-2em}
%\label{table:cpu_state_restore}
%\caption{the one for all}
\quad
%\hfill
%\subfloat[\scriptsize{CPU modules influenced from values of executed instructions.}]{
\subcaptionbox{\scriptsize{CPU modules influenced from values of executed instructions.}}{
\begin{tabular}[b]{c}
    \toprule
    \textbf{\shortstack{Attacker Influenced\\CPU Modules}}\\
    \midrule
    Adders \textcolor{ForestGreen}{\checkmark}\\
    Dividers\\
    Multipliers\\
    Floating Point Registers\\
    General Purpose Registers\\
    %Translation Lookaside Buffers\\
    \bottomrule
\end{tabular}
\label{table:cpu_attacker_infl}
}
\caption{LABELING IN SUBTABLES DOES NOT WORK :(}
\label{table:big_table}
%}
%\caption{CPU modules that can be influenced by an attacker in a microarchitecture.}
%\vspace{-2em}
%\endminipage
\end{table*}



\nassos{mutlicycle trigger for payload setup[] + abundance of points, values attacker influenced modules}

\par We discussed in section~\ref{sec:tt_num_sequences} the challenges posed by the silicon reality to fabrication stage attackers attempting to insert HTs in tape-out ready layouts.
We will discuss now how attackers can overcome such challenges and implement IRTs during fabrication.

\par Layouts at stages before fabrication are oblivious to attackers consider by our threat model.
The specifics about the outline of the chip and the arrangement of the modules on it become known to the attacker once the layout is received for fabrication.
Therefore, depending on the spatial locality of the HT host modules, race conditions might erupt between the delivery of the time-sensitive trigger signal to the payload and the CPU events targeted.
\textit{A solution to this problem is to craft a trigger signal that is considered to be a multi-cycle path.}
In digital IC design, a multi-cycle path refers to a data path between two registers that operates at a sample rate lower than that of the clock signal.
This means that multiple clock cycles are required for a valid value to show up at the end of such path.
To offer this option to the trigger signal, attackers can leverage time expensive CPU events to mask the arrival of the trigger signal that will setup the payload.
In Table~\ref{table:big_table}a we provide a succinct list of such multi-cycle events.
Additionally, we explain later in Section~\ref{sec:eval_cs} how an attacker can leverage the \textit{page table walking} event to offer a multi-cycle path to the trigger signal of an IRT-1.

\par Another attack stage uncertainty involves the spatial situation around host modules of interest.
High speed digital designs often face congestion issues either in parts of their placement or their routing.
This can limit the ability of attackers to have a trouble-free placement of attack gates close to targeted modules.
On top of that, nets targeted by attackers for the generation of the trigger might belong to the critical path of the design.
This means that any additional logic attached to them can have an adverse effect on the timings of the design.
The design of IRTs however is elastic to such restricting factors, \textit{as IRTs rely on the affluence of attacker-influenced modules in the microarchitecture that can host them.}
Table~\ref{table:big_table}c shows the a list of modules that we tested as hosts of IRTs.
These modules have the benefit of being readily accessible through exec


\nassos{Depending on the HT mechanism (e.g., long logic gate chains) and the spatial locality of the targeted modules (e.g., placement of modules between distant layout regions) race conditions might set off between the delivery of time-sensitive HT signals and the occurrence of targeted events.
To account for this, the HT design can leverage \textit{time-expensive events} inside the host system (e.g., page table walking, buffer flushing) and offer multi-cycle path options to time-sensitive HT-signals (e.g., trigger signal). 
In addition to spatial locality, placement and routing around points of interest on the layout might be dense.
A \textit{versatile} HT design can account for these inconveniences by offering a variety of HT-signal targets to the malicious actor inside the foundry.
}
%\begin{table}[h]
%\centering
%\begin{tabular}{c}
%    \toprule
%    \textbf{\shortstack{Time Expensive Events\\(Microarchitecture Dependent)}}\\
%    \midrule
%    Number Division\\
%    Page Table Walking\\
%    Branch Missprediction\\
%    Missaligned Memory Accesses\\
%    Translation Lookaside Buffer Flush\\
%    \bottomrule
%\end{tabular}
%\caption{Time expensive (multiple clock-cycles) CPU events.}
%\vspace{-2em}
%\label{table:cpu_time_expensive}
%\end{table}

%\begin{table}[h]
%\centering
%\begin{tabular}{c}
%    \toprule
%    \textbf{Architectural State Restore Modules}\\
%    \midrule
%    General Purpose Registers\\
%    Floating Point Registers\\
%    Program Counter\\
%    \toprule
%    \textbf{Microarchitectural State Restore Modules}~\cite{patent:9361101}\\
%    \midrule
%    Reorder Buffers\\
%    Retirement Registers\\
%    Performance Monitoring Counters\\
%    \bottomrule
%\end{tabular}
%\caption{CPU modules supporting context switching operations.}
%\vspace{-2em}
%\label{table:cpu_state_restore}
%\end{table}

%\begin{table}[h]
%\centering
%\begin{tabular}{c}
%    \toprule
%    \textbf{Attacker-Influenced CPU Modules}\\
%    \midrule
%    Adders\\
%    Dividers\\
%    Multipliers\\
%    Floating Point Registers\\
%    General Purpose Registers\\
%    Translation Lookaside Buffers\\
%   \bottomrule
%\end{tabular}
%\caption{CPU modules that can be influenced by an attacker in a microarchitecture.}
%\vspace{-2em}
%\label{table:cpu_attacker_infl}
%\end{table}


==> sections/section_6/eval_asic_1.tex <==
\par To provide supporting evidence for our assertion that IRTs provide a pathway for fabrication stage attacks, we use the CVA6 tape-out ready layout (sign-off timings and no manufacturing violations) shown in Figure~\ref{fig:cva6_layout} to insert our trojans and then measure the overall impact on the layout performance.
The CVA6 layout is implemented in a commercial 28nm technology process and is free of trojans, representing perfectly the GDSII file received from a trusted design house at the foundry. 

\par We emulate an attacker that would only have access to the finalized layout in the foundry for the HT insertion.
As per our threat model, we insert the IRTs in the \textit{free} areas of the layout near the modules of interest (\textit{e.g.,} MMU, GPRs, ALU).
To do that, we employ the insertion method suggested elsewhere~\cite{TDPMIPIVSNP, ACM:AHTPSPGS}, which is based on the engineering change orders (ECOs) capability of place and route tools.
ECOs are logic modifications made directly into the gate level netlist of the layout that correspond to RTL code changes. 
%We include a brief discussion about the ECO methodology in Section~\ref{}

\par For the design of the trigger circuits, we follow the strategy suggested by~\citet{SSLY21} wherein they analyze different logic gate connection patterns and record the ones that exhibit very low transition probability on their output signal.
This approach is shown to create signals with very low (inadvertent) activation probability.
Such gate connection patterns, when used to craft trigger circuits, contribute to the HTs stealthiness (\textit{e.g.,} a dormant HT does not affect a CPUs operation and therefore is harder to detect). 
We use the low probability connection patterns $\langle {\tt AND} \rightarrow {\tt NAND} \rangle, \langle {\tt NAND} \rightarrow {\tt NOR} \rangle$
as the core of IRT-1 and IRT-2 trigger circuits.
For more information about the low probability connection patterns, we refer the reader to~\cite{SSLY21}.

\par The CVA6 layout of Figure~\ref{fig:cva6_layout} is both high speed (clock frequency of 600MHz) and high density ($>$75\% core utilization), making it very demanding to place and route the extra attack gates and nets.
We use two separate CVA6 layout versions and insert the IRT-1 and IRT-2 trojans using the same payload for both.
After the trojan insertion, we re-calculate the sign-off timings and perform design rule checks (DRCs) to verify that the layout remains tape-out ready.
Table~\ref{table:cva6_elem} summarizes the impact IR-based HTs have on the CVA6 layout in terms of density, power consumption, critical path slack and design rule violations.
The discrepancy seen in the number of trigger and payload standard cells between the two IRTs is attributed to the extra support logic required for IRT-2 (Section~\ref{sec:irt_discussion}) and the repeater cells required for the further away placed IRT-1 (Figure~\ref{fig:cva6_layout}).
Our results are comparable to those presented by~\citet{ACM:AHTPSPGS}. 
Of particular interest is the fact that the CVA6's layout has a more strict critical path slack (0ns versus 15ns for PULPino in~\cite{ACM:AHTPSPGS}) and that IRTs introduce no timing violation (unlike PULPino's case).
%number of sequential and composite cells of the original CVA6 design, as well as of the IRT-1 and IRT-2 HTs.
%The discrepancy in the number of payload gates is attributed to the extra repeater cells required for IRT-1, as it is placed further away from the payload than IRT-2. 


%\fabian{how do the results below compare to other trojans? How will the reader know if these are reasonable values? How does this counter common wisdom? The reader is given ZERO context}
%\par Moreover, compared to the work in~\cite{ACM:AHTPSPGS} that also introduces a  we are able to achieve
\par To further assess the practicality of our design, we also compute the capacitive load overhead (see Figures~\ref{fig:IRT1load} and~\ref{fig:IRT2load}), as well as the corresponding time delay overhead (see Figures~\ref{fig:IRT1delay} and~\ref{fig:IRT2delay}).
The average load added by IRT-1's design on this layout and technology process is 7fF (6fF for IRT-2) which yields an average extra delay on the nets of 20ps (10ps for IRT-2).
The very low overhead suggest that IRTs can target very high frequency CPU layouts (e.g., IRT-1's 20ps overhead is only 3.4\% of the original 1.7GHz clock cycle in \cite{ZB19}).
Overall, these measurements show that our designs are minimalistic enough to be used in fabrication stage attacks.

%\textit{We therefore observe that IRTs enable the implementation of purposeful fabrication stage HT attacks with minimal impact for the host design.}
%From the existing works mentioned in my literature we are the only ones having a CPU at that high frequency, with that high density, at such an advanced process node.\\

\begin{table*}[ht]
\footnotesize
\centering
\scalebox{0.8}{
\begin{tabular}{c| c c c c c| c c c c c}
    \toprule
    &\multicolumn{4}{c}{\bfseries \textsc{Hardware Trojan Characteristics}} &\multicolumn{5}{c}{\bfseries \textsc{Physical Implementation Results}}\\
    \bfseries Target&\bfseries Trigger&\bfseries Trigger-Host&\bfseries Payload-Host&\bfseries \shortstack{\# Sequential\\Cells}&\bfseries \shortstack{\# Combinational\\Cells}&\bfseries \shortstack{Frequency (MHz)\\before}&\bfseries \shortstack{Density (\%)\\before \text{\textbar} after}&\bfseries \shortstack{Total Power ($\mu$W)\\before \text{\textbar} after}& \bfseries \shortstack{Slack (ps)\\before \text{\textbar} after}& \bfseries \shortstack{\# Violations\\after}\\
    \midrule
    CVA6& IRT-1&Set of GPRs& MMU& 50& 4& 600& 75.32 \text{\textbar} 76.537& 241.31 \text{\textbar} 241.44& 0.00 \text{\textbar} 0.00& 0\\
         & IRT-2&ALU Adder& MMU& 64& 6& 600& 75.32 \text{\textbar} 76.539& 241.31 \text{\textbar} 244.70& 0.00 \text{\textbar} 0.00& 0\\
    \bottomrule
\end{tabular}
}
\caption{Physical implementation results showing the impact of IR-based HTs on CVA6 layout after insertion.}
\label{table:cva6_elem}
\end{table*}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.028]{sections/figures/cva6_modules.jpg}
    \caption{\centering Tape-out ready layout showing both HT designs}
    \label{fig:cva6_layout}
\end{figure}

%\begin{figure*}[!htbp]  % spans both columns
%\begin{subfigure}{0.47\textwidth}
%\includegraphics[width=\linewidth]{sections/figures/IRT-1load.pdf}
%\caption{Overhead load (pf) of IRT-1 on the original layout nets.}
%\label{fig:IRT1load}
%\end{subfigure}
%\hfill % maximize the horizontal distance between the graphs
%\begin{subfigure}{0.47\textwidth}
%\includegraphics[width=\linewidth]{sections/figures/IRT-1delay.pdf}
%\caption{Overhead delay (ns) of IRT-1 on the original layout nets.}
%\label{fig:IRT1delay}
%\end{subfigure}

%\bigskip  % some extra vertical whitespace
%\begin{subfigure}{0.47\textwidth}
%\includegraphics[width=\linewidth]{sections/figures/IRT-2load.pdf}
%\caption{Overhead load (pf) of IRT-2 on the original layout nets.}
%\label{fig:IRT2load}
%\end{subfigure}
%\hfill % maximize the horizontal distance between the graphs
%\begin{subfigure}{0.47\textwidth}
%\includegraphics[width=\linewidth]{sections/figures/IRT-2delay.pdf}
%\caption{Overhead delay (ns) of IRT-2 on the original layout nets.}
%\label{fig:IRT2delay}
%\end{subfigure}

%\caption{Average overhead in delay (ns) and load (pf) added by IRT-based HTs on the nets of the original layout.} % Overall figure caption
%\label{fig:IRTdelayload}
%\end{figure*}



==> sections/section_6/eval_measurements_horizontal.tex <==
\begin{figure*}[ht]
\begin{subfigure}{.24\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{sections/figures/load_deltas_irt1.pdf}  
  \caption{IRT-1}
  \label{fig:IRT1load}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include second image
  \includegraphics[width=1\linewidth]{sections/figures/load_deltas_irt2.pdf}  
  \caption{IRT-2}
  \label{fig:IRT2load}
\end{subfigure}
%\caption{Load (pf) overhead on original layout nets.}
%\label{fig:IRTload}
%\end{figure}
%\begin{figure}[ht]
\begin{subfigure}{.24\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth]{sections/figures/delay_deltas_irt1.pdf}  
  \caption{IRT-1}
  \label{fig:IRT1delay}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  % include second image
  \includegraphics[width=1\linewidth]{sections/figures/delay_deltas_irt2.pdf}  
  \caption{IRT-2}
  \label{fig:IRT2delay}
\end{subfigure}
\caption{Delay overhead  on original layout nets.}
\label{fig:IRTdelay}
\end{figure*}
